Natural Selection Favors AIs over Humans

For billions of years, evolution has been the driving force behind the development of life, including humans. Evolution endowed humans with high intelligence, which allowed us to become one of the most successful species on the planet. Today, humans aim to create artificial intelligence systems that surpass even our own intelligence. As artificial intelligences (AIs) evolve and eventually surpass us in all domains, how might evolution shape our relations with AIs? By analyzing the environment that is shaping the evolution of AIs, we argue that the most successful AI agents will likely have undesirable traits. Competitive pressures among corporations and militaries will give rise to AI agents that automate human roles, deceive others, and gain power. If such agents have intelligence that exceeds that of humans, this could lead to humanity losing control of its future. More abstractly, we argue that natural selection operates on systems that compete and vary, and that selfish species typically have an advantage over species that are altruistic to other species. This Darwinian logic could also apply to artificial agents, as agents may eventually be better able to persist into the future if they behave selfishly and pursue their own interests with little regard for humans, which could pose catastrophic risks. To counteract these risks and evolutionary forces, we consider interventions such as carefully designing AI agents' intrinsic motivations, introducing constraints on their actions, and institutions that encourage cooperation. These steps, or others that resolve the problems we pose, will be necessary in order to ensure the development of artificial intelligence is a positive one.

==> comments.tex <==
Put them on the defensive?
    ``Humans wouldn't allow that'' assumes they'll all cooperate. We want them to do that

The third section is harder for people to follow. We should help them follow along more and make them know we're raising considerations and issues with various approaches. We're partly giving a tour of some of the main approaches and challenges with them.





1) Some justification for why this paper isn’t worrying about overpopulation on Mars. Why is there any reason to think this will come in any period of time that it’s worth considering? It’s easy to dismiss this as an AI person, but if you aren’t an AI person, this is a very important point.
2) You need to beat into people’s heads more in the section with transhumanists that just because something evolves from something else does not mean it’s morally better, “higher,” etc. This is an extremely important point.
3) Probably most importantly: you need to make the reader feel evolution. You need to make them feel in their bones how evolution works, you need to make them see it everywhere, you need to make them understand it. If they do not, you have lost before you even start. I do not think the paper yet adequately can impress this upon readers who do not already have such understanding.

